PD-ML-Lite: Private Distributed Machine Learning from Lighweight Cryptography

Privacy is a major issue in learning from distributed data. Recently the cryptographic literature has provided several tools for this task. However, these tools either reduce the quality/accuracy of the learning algorithm---e.g., by adding noise---or they incur a high performance penalty and/or involve trusting external authorities. We propose a methodology for {\sl private distributed machine learning from light-weight cryptography} (in short, PD-ML-Lite). We apply our methodology to two major ML algorithms, namely non-negative matrix factorization (NMF) and singular value decomposition (SVD). Our resulting protocols are communication optimal, achieve the same accuracy as their non-private counterparts, and satisfy a notion of privacy---which we define---that is both intuitive and measurable. Our approach is to use lightweight cryptographic protocols (secure sum and normalized secure sum) to build learning algorithms rather than wrap complex learning algorithms in a heavy-cost MPC framework. We showcase our algorithms' utility and privacy on several applications: for NMF we consider topic modeling and recommender systems, and for SVD, principal component regression, and low rank approximation.

==> privacy_analysis_svd.tex <==
% !TEX root = ../PD-SVD.tex
%\label{sec:ksdp}

In the context of protecting privacy in a multiparty computation, it is appropriate to study the privacy of individual rows of each party's database~\cite{kairouz2016fundamental}. 
Informally, Distributional Differential Privacy (DDP) aims to achieve similar guarantees as DP but without necessarily using external noise in the mechanism; instead uncertainty about the data is used to conceal the relevant information.
%As a result one does not necessarily need the external noise, which, as said, might perturb the output of the learning process in an unquantifiable manner. 
More concretely, in Distributional Differential Privacy, e.g.~\cite{bassily2013coupled,groce2014new}, a mechanism $\mathcal A$ is said to be ``distributionally differentially private'' 
for dataset $X$ drawn from sampling distribution $\mathcal D$, and all individual rows $x\in X$ if there exists some mechanism $\mathcal B$ such that
%\begin{equation*} P[\mathcal A(X)] \approx P[\mathcal B(X\setminus\{x\})],
%\end{equation*}
\[
P[\mathcal A(X)] \approx_{\epsilon, \delta} P[\mathcal B(X\setminus\{x\})].
\]
For probability density functions $f,g$
over sample space $\Omega$ with sigma-algebra $\mathcal S \subseteq 2^\Omega$,
$f\approx_{\epsilon, \delta}g$ if
\begin{equation}
\begin{aligned}
\forall \omega \in \mathcal S\, f(\omega) &\leq e^\epsilon g(\omega)+\delta\\
\text{ and } g(\omega) &\leq e^\epsilon f(\omega)+\delta.
\end{aligned}
\label{eq:ddp}
\end{equation}

Consider the simulator $\mathcal B$ that simply draws a new database from the distribution $\mathcal D$, and then runs $\mathcal A$. If $P[\mathcal A(X)]~\approx~P[\mathcal A(\mathcal D)]$, then mechanism $\mathcal A$ doesn't reveal anything about database $X$ other than what can be inferred from the underlying distribution $\mathcal D$.

To define the sample-space $\Omega$ in an $M$-party computation, we need to define the concept of an {\it observable}.\\

\centerline{\fbox{\parbox{0.925\columnwidth}{
\textbf{Observable.}
Suppose a distributed mechanism $\mathcal A$ is executed among several parties. The party of interest uses database a $X$, while the concatenation of the remaining parties' databases is $Y$. Then $\mathcal O_{\mathcal A, X, Y}$ is the set of all objects that a coalition of adversaries observes from the communication transcript of $\mathcal A$.
}}}

Therefore a mechanism $\mathcal A$ can be interpreted to satisfy distributional privacy for document $x$ if it can be simulated by a mechanism $\mathcal B$. Where $\mathcal B$ must operate without access to $x$ but still emit {\it all} observables $\mathcal O_{\mathcal A, X,Y}$ with a comparable probability distribution to $\mathcal A$.

The easiest way to satisfy such a strict privacy requirement for all observables is to build mechanism $\mathcal A$ using differential privacy.
As we discussed in the Introduction, the benefit one gets with using differential privacy is that privacy is guaranteed against a large class of post-processing.%, i.e. adversaries with super-polynomial computational power and unlimited auxiliary information.
 The cost of such a strong guarantee is that it's difficult to predict the effect that differential privacy will have on the quality of the SVD.
Since we want to reconstruct the centralized SVD exactly, this weakness is a the main reason why we don't used DP.
Furthermore, because of economic incentives, for many applications is unnecessary to be protected against an arbitrarily powerful adversary.

%,wang2015privacy}.
%However the loss in learning accuracy is difficult to quantify. Theoretical results in \cite{balcan2012distributed} give estimates for the number of samples needed to match centralized learning error plus/minus some tolerance for given $\epsilon,\delta$ for simple mechanisms. But what happens to the learning outcome when an algorithm is constructed out of the composition of these simple mechanisms needs to be examined on case-by-case basis, and things get ugly as the tolerance goes to 0. More concretely, in one-party Differentially Private NMF~\cite{FastDPMF} the authors observe a 19\% loss in learning quality (RMSE in their case) when strict DP is satisfied even for $\epsilon=0.25$. In order to improve the learning outcome, they propose violating privacy guarantees for atypical users. This lets them use a smaller $\epsilon$ and lets them add less noise to the mechanism, similar to how we increased $\delta$ for the one bit sum example.

%Most differential privacy efforts have been focused on the one-party setting.
%Here a curator has access to the data and is trying to answer queries in a differentially private manner.
%However in our setting there are $M$ parties co-operating to answer `a query.'
%This task is much more challenging is now the parties are also interested in protecting intermediate results from one another.
%As a result, due to a possible difference attack on observables at iteration $i$ and $i+1$ it is necessary for each party to add noise to all observables they emit for every iteration~\cite{rajkumar2012differentially, hua2015differentially}. In Section~\ref{sec:learning_outcomes} we will examine the potential effect of adding noise at every iteration for NMF and SVD.

A adversary limited to polynomial computation is limited by the curse of dimensionality.
%Privacy as defined by Equation \ref{eq:ddp} is often not computationally tractable.
The fundamental issue is that the volume of the sample space from which observables $\mathcal O$ are drawn grows exponentially in $d$. A standard result in probability density estimation states that expected square error for the probability density decreases at a rate of $O(n^\frac{1}{d})$~\cite{hansen2009lecture}. This means that an adversary with polynomial computation power cannot reliably identify an outcome $\omega \in \mathcal S$ as indicative of the absence or presence of a particular document $x$, because this adversary doesn't have an accurate estimate for $P[\omega]$. Even if the adversary could estimate $P[\omega]$, they would still face the issue that $\mathcal S$ is exponentially large, which makes it difficult to find non-private $\omega$ in this space.

%For these reasons we define an alternative (to Equation \ref{eq:ddp}) experimentally verifiable notion of distance based on statistics of the observables.
Therefore we make the assumption that economically-constrained adversaries will reason about distributions of statistics of observables, rather than distributions of the observables themselves.
Let $s \colon \mathcal O \times x \to \R$ be a document-dependent statistic.
%We want to compare probabilities of subsets of subsets of the sample space. However since any finite sample of observed statistic values will have 0 probability under a continuous distribution, we almost surely end up with $\epsilon=0$ and $\delta>0$ in Equation \ref{eq:ddp}. Therefore, in practice we need to consider $\delta$, which corresponds to the $\ell_1$ distance between PDFs. However, estimating PDFs is difficult; but by estimating the $\ell_1$ distance between CDFs we capture the spirit of Equation \ref{eq:ddp}, while making the computational problem much easier.
Within the context of a statistic $s$ and a document $x$, let $f$ be the distribution of $\sigma$ with observables $\mathcal O_{\mathcal A, X,Y}$ and $g$ by the distribution of $\sigma$ with observables $\mathcal O_{\mathcal B,X\setminus\{x\},Y}$ (i.e. those emitted by a simulator $\mathcal B$ which doesn't have access to $x$).
Equation \ref{eq:ddp} proposes one way of defining the similarity between PDFs $f$, and $g$. However Equation \ref{eq:ddp} is both difficult to satisfy, and unnecessarily strict for protecting against polynomial-compute adversaries. Since the spirit of distributional privacy is maintained under other notions of similarity between distributions (however useful properties like composition are lost) we look elsewhere.
In particular, instead of attempting to measure the similarity between PDFs $f$ and $g$ we propose measuring similarity between the corresponding CDFs $F$ and $G$ using the well-known Kolmogorov-Smirnov statistic.
%For any finite sample of statistic values drawn from $f$ (resp. $g$) the probability assigned to those values under a continuous $g$ (resp. $f$) will be 0 almost surely. As a result in order to satisfy Equation \ref{eq:ddp} we will have $\epsilon=0$ and $\delta>0$. Therefore, in practice we need to consider $\delta$, which corresponds to the $\ell_1$ distance between the PDFs $f$ and $g$. However, estimating PDFs is difficult; but by estimating the $\ell_1$ distance between CDFs we capture the spirit of Equation \ref{eq:ddp}, while making the computational problem much easier.
%Privacy can be achieved in the distributional sense~\cite{bassily2013coupled} if $F\approx G$.
It is defined for empirical CDFs $F, G$ that have support on an interval $[a,b]$ as
\mldc{\text{KS}(F,G)\equiv\sup_{x\in[a,b]} |F(x) - G(x)|.}
This statistic can then be used in the Kolmogorov-Smirnov 2-sample hypothesis test, which outputs a $p$-value that represents the probability that a statistic at least as extreme as the one observed would be drawn if $F$ and $G$ were sampled from the same underlying distribution.
Now we are ready to define our version of distributional privacy.

\centerline{\fboxsep5pt\fbox{\parbox{0.925\columnwidth}{
\textbf{KS Distributional Privacy ($\pi$-\ksdp).}
A mechanism $\mathcal A$ satisfies $\pi$-KS Distributional Privacy if there exists a simulator mechanism $\mathcal B$ such that
for all statistics $s\in\{s_1, s_2,\ldots\}$,
and for all documents $x\in~X$,
the KS 2-sample test run on ECDF($s(\mathcal O_{\mathcal A, X,Y},x)$) and ECDF($s(\mathcal O_{\mathcal B, X\setminus \{x\},Y},x)$) returns $p\geq \pi$.
}}}
%\\[2pt]

In words, \ksdp means that the observables generated by a simulator $\mathcal B$ that doesn't have access to a document $x$ cannot be statistically distinguished from the actual algorithm $\mathcal A$ running on the database with $x$ included.

The KS-test's $p$-value is simply used as a measure of distance between two distributions which takes number of samples into account.
A high $p$-value means that we cannot reject that the two ECDFs are the result of sampling from the same underlying distribution.
It doesn't mean that we can conclude they come from the same distribution.
Although hypothesis tests with the reverse null/alternate hypothesis have been studied~\cite{wellek2010testing}, computational efficiency and interpretability are significant challenges. Important future work is to examine methods for distinguishing distributions.

%Also, there are computational benefits for defining similarity between distributions using the CDFs.
%The primary reason is that due to the DKW Inequality~\cite{massart1990}, the error in the statistic $(F,G)$ is $O(e^{-n})$, i.e. it decays exponentially in the number of samples.
%Meanwhile the mean integrated square error in estimates of the probability density function are $O(n^{-0.8})$, which has sub-linear decay.
%As a result it requires fewer samples to estimate with high confidence the extent to which two observables are statistically indistinguishable when using measures based on the CDFs, than it is when using measures based on the PDFs, such as Equation~\ref{eq:ddp}.

\begin{algorithm}[t]
\caption{Measuring $\pi$-\ksdp.\vnote{This algorithm is different than the one in PD-NMF is there a reason? Which one should we keep? }}
\label{alg:posterior_test}
\floatname{algorithm}{Procedure}
\begin{algorithmic}[1]
%\fontsize{6.5pt}{7.5pt} \selectfont %Assuming ICML2018 doesnt allow reduced algorithm fonts
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\Require Mechanism $f$, set of statistics $S$, database $X$, document of interest $x$, number of samples per document $t$.
\Ensure Minimum $p$-value for all statistics.
\State Determine what the \termdef{observables} of $f$ are.
%\State Propose informative statistics $\Sigma$
\State Generate database sub-samples $\{X'_i\}_{i=1}^t$,  $X'_i \subseteq X$
\State Evaluate the mechanism $f(X'_i \cup \{x\})$ for all $i$.
\State Generate d.b. sub-samples $\{Y_i\}_{i=1}^t$,  $Y_i\subseteq X\setminus  \{x\}$
\State Evaluate the mechanism $f(Y_i)$ for all $i$.
\State Set $\pi \gets 1$
\For{each $s \in S$}:
\State w/ $\gets$ ECDF(\{$s(f(X_i), x)\}_{i=1}^t$).
\State w/o $\gets$ ECDF($\{s(f(Y_i),x)\}_{i=1}^t)$.
\State $p \gets $ KS 2 sample test on w/ and w/o.
\State $\pi \gets \min(p,\pi)$
\EndFor\\
\Return $\pi$
\end{algorithmic}

\end{algorithm}
The definition of $\pi$-\ksdp leads to a
method for measuring the privacy of a distributed mechanism,
presented as Algorithm~\ref{alg:posterior_test}.
For the simulator mechanism, we simply run $\mathcal A$ on a database randomly generated from the underlying distribution $\mathcal D$ with the only restriction being that the particular document $x$ isn't included.
A weakness of $\pi$-\ksdp is that it doesn't guarantee
future-proof privacy against new statistics and auxiliary information.
Rather it tests whether a given set of statistics is discriminative enough to break distributional differential privacy.
An advantage of Algorithm \ref{alg:posterior_test} is that samples can be generated, stored, and re-used to test many different statistics quickly.
Furthermore, Algorithm \ref{alg:posterior_test} is suitable as a defensive algorithm for identifying sensitive documents $x$, which can be excluded from distributed learning if need be.
%Effective simulators $\mathcal B$ are to run $\mathcal A$ but either replace $x$ by a random document, or sample $n$ random documents to create an entirely new database.
In Section~\ref{sec:experimental_results} we use Algorithm~\ref{alg:posterior_test} to give evidence that \pdsvd satisfies $\pi$-\ksdp.
